Learning Answer Generation using Supervision from Automatic Question Answering Evaluators

Recent studies show that sentence-level extractive QA, i.e., based on Answer Sentence Selection (AS2), is outperformed by Generation-based QA (GenQA) models, which generate answers using the top-k answer sentences ranked by AS2 models (a la retrieval-augmented generation style). In this paper, we propose a novel training paradigm for GenQA using supervision from automatic QA evaluation models (GAVA). Specifically, we propose three strategies to transfer knowledge from these QA evaluation models to a GenQA model: (i) augmenting training data with answers generated by the GenQA model and labelled by GAVA (either statically, before training, or (ii) dynamically, at every training epoch); and (iii) using the GAVA score for weighting the generator loss during the learning of the GenQA model. We evaluate our proposed methods on two academic and one industrial dataset, obtaining a significant improvement in answering accuracy over the previous state of the art.

==> [ACL'23] Automatic QA Evaluator-Supervised Answer Generation/plot/ablation_baseline_vs_avaweight_on_avascore.tex <==


\begin{figure}[t]
    \begin{tikzpicture}
    \begin{axis} [
        width=0.95\linewidth, 
        xlabel=Epochs, 
        ylabel=GAVA-Score, 
        legend style={at={(1,0)},anchor=south east}
    ]
    \addplot table [x=epoch,y=baselineavascore, col sep=comma] {data.csv};
    \addplot table [x=epoch,y=avaweightavascore,col sep=comma] {data.csv};
    \legend {GenQA-WS,AVA-LW};
    \end{axis}
    \end{tikzpicture}
    \vspace{-0.5em}
\caption{Comparison of baseline GenQA-WS and AVA-LW on WQA in terms of GAVA-Score (on validation split) varying across training epochs (GAVA-LW achieves higher GAVA-Score throughout training).}
\label{fig:ablation_avascore_ws_vs_avalw}
\end{figure}

==> [ACL'23] Automatic QA Evaluator-Supervised Answer Generation/plot/ablation_sda_with_different_thresholds.tex <==

\begin{figure}
\begin{tikzpicture}
\begin{axis} [
    width=0.9\linewidth, 
    ymin=0.79,
    xlabel=Epochs, 
    ylabel=GAVA-Score, 
    legend style={at={(1,0)},
    anchor=south east}
    ]
    \addplot table [x=epoch,y=th05,col sep=comma] {ablationthresh.csv};
    \addplot table [x=epoch,y=th07,col sep=comma] {ablationthresh.csv};
    \addplot table [x=epoch,y=th09,col sep=comma] {ablationthresh.csv};
    \legend {$\theta{=}0.5$,$\theta{=}0.7$,$\theta{=}0.9$};
\end{axis}
\end{tikzpicture}
\vspace{-0.8em}
\caption{Comparison of three different GAVA-SDA models trained on MS-MARCO using different thresholds $\theta$ in terms of GAVA-Score (on validation split) varying across training epochs. The model trained with the largest value of $\theta$ achieves the highest GAVA-Score.}
\label{fig:ablation_thresholds}
\vspace{-0.3em}
\end{figure}
